Congestion Control Mechanisms in IEEE 802.11p and Sidelink C-V2X

Connected vehicles are expected to play a major role in the next future to improve safety and traffic efficiency on the road and short-range technologies have been defined to enable the direct exchange of information. To this aim, two solutions are currently the subject of a debate that goes beyond the technician, i.e., IEEE 802.11p and sidelink cellular-vehicle-to-anything (C-V2X). Tested and mature for deployment the first, possibly more efficient the second. In both cases, one of the main aspects is the management of channel congestions, which can cause serious packet losses and have a critical impact on the reliability of applications. Congestions can be managed through different approaches, including the control of transmission power, packet generation frequency, and the adopted modulation and coding scheme. Congestion management has been well studied in IEEE 802.11p, with consolidated algorithms included in the standards, whereas it appears somehow as a new topic looking at C-V2X. In this work, a review of the main congestion control mechanisms and a discussion of their applicability and efficiency in the two technologies is provided. This topic is addressed without focusing on specific algorithms and with the aim to provide general guidelines as a starting point for new proposals.

==> Table11p.tex <==
\begin{table}%[!t]
\caption{IEEE 802.11p modulation and coding schemes and corresponding values.
\vspace{-2mm}
\label{Table:11pMCS}}
\scriptsize
\centering
\begin{tabular}{p{1cm}p{2.2cm}p{1.5cm}p{1.6cm}p{1.6cm}p{1.4cm}}
\hline
\textbf{MCS \#} & \textbf{Modulation, coding rate} &  \textbf{Gross rate (Mb/s)}  & \textbf{Minimum SINR~[dB]} &  \textbf{Range [m] (only~PL)} & \textbf{Duration [$\mu$s]} \\  
%\hline 
%\\
1 & BPSK, 1/2 & 3.0 & 10.0 & 223 & 848 \\ 
2 & BPSK, 3/4 & 4.5 & 11.0 & 210 & 584 \\ 
3 & QPSK, 1/2 & 6.0 & 13.0 & 188 & 448 \\ 
4 & QPSK, 3/4 & 9.0 & 15.0 & 167 & 312 \\ 
5 & 16QAM, 1/2 & 12.0 & 18.0 & 141 & 248 \\ 
6 & 16QAM, 3/4 & 18.0 & 22.0 & 112 & 176 \\ 
7 & 64QAM, 2/3 & 24.0 & 26.0 & 89 & 144 \\ 
8 & 64QAM, 3/4 & 27.0 & 27.0 & 84 & 136 \\ 
\hline%\multicolumn{3}{c}{\textbf{\textit{Common settings}}} \\ \hline
\end{tabular}
%\vskip 0.5cm
\end{table}


==> TableLTE.tex <==

\begin{table}[t!]
\caption{LTE-V2X modulation and coding schemes and corresponding values. \vspace{-2mm}
\label{Table:LTEMCS}}
%\scriptsize
%\footnotesize
%\small
\centering
%\begin{tabular}{p{0.6cm}|p{1cm}p{0.8cm}p{1.2cm}p{0.5cm}p{0.9cm}p{0.7cm}}
\begin{tabular}{p{1cm}p{1.8cm}p{0.6cm}p{1.4cm}p{1.5cm}p{1.0cm}p{0.9cm}}
\hline
%\textbf{300~B} & & & & & \textbf{Configuration} \\
\textbf{MCS \#} & \textbf{Modulation, Coding rate}  &
\textbf{RB Pairs} &\textbf{Min. SINR~[dB]} & \textbf{Range [m] (only~PL)}  & \textbf{Subch. size}&
\textbf{Packets per~TTI}\\  
%\hline
0 & QPSK, 0.13 & 86	& -2.83	& 418 & 5 & - \\ 
1 & QPSK, 0.17 & 66 & -1.38 & 411 & 5 & -\\ 
2 & QPSK, 0.21 & 54 & -0.22 &  404 & 5 & -\\ 
3 & QPSK, 0.27 & 41 & 1.49 & 392 & 5 & 1\\ 
4 & QPSK, 0.33 &34	& 2.76 & 382 & 6 &	1\\ 
5 & QPSK, 0.41 & 28 & 4.40 & 365 & 5	& 1 \\ 
6 & QPSK, 0.48 & 23 & 5.79 & 354 & 5 & 2 \\ 
7 & QPSK, 0.57 & 20 & 7.30 & 336 & 6 & 2  \\ 
8 & QPSK, 0.65 & 18 & 8.60 & 320 & 5 &	2 \\ 
9 & QPSK, 0.73 & 16 & 9.88 & 306 & 6 & 2  \\ 
10 & QPSK, 0.82 & 14 & 11.16 & 294 & 6 & 2 \\ 
11 & 16QAM, 0.41 & 14 & 11.16 & 294 & 6 & 2 \\
12 & 16QAM, 0.46 & 12 &12.83 &  278 & 5 &	3  \\ 
13 & 16QAM, 0.52& 11& 14.46 & 258 & 5 &	3 \\
14 & 16QAM, 0.59 & 10 & 16.39 &	237 & 6 &	4  \\  
15 & 16QAM, 0.67 & 9 & 18.73 & 213 & 6 & 4  \\ 
16 & 16QAM, 0.72 & 8 & 20.05 & 203 & 5 &	5 \\
17 & 16QAM, 0.75 & 8 & 21.10 & 191 & 5 &	5 \\ 
18 & 16QAM, 0.84 & 7 & 23.54 & 172 & 5 &	5 \\
19 & 16QAM, 0.92 & 7 & 25.93 & 150 & 5 &	5 \\
20 & 16QAM, 1.00 & 6 & 28.10 & 137 & 5 &	5 \\ 
\hline
%\multicolumn{3}{c}{\textbf{\textit{Common settings}}} \\ 
\end{tabular}
%\vskip 0.5cm
\end{table}

